Density of small singular values of the shifted real Ginibre ensemble

We derive a precise asymptotic formula for the density of the small singular values of the real Ginibre matrix ensemble shifted by a complex parameter $z$ as the dimension tends to infinity. For $z$ away from the real axis the formula coincides with that for the complex Ginibre ensemble we derived earlier in [arXiv:1908.01653]. On the level of the one-point function of the low lying singular values we thus confirm the transition from real to complex Ginibre ensembles as the shift parameter $z$ becomes genuinely complex; the analogous phenomenon has been well known for eigenvalues. We use the superbosonization formula [arXiv:0707.2929] in a regime where the main contribution comes from a three dimensional saddle manifold.

==> packages.tex <==
\usepackage[english]{babel}
\usepackage[p,osf]{cochineal}
\usepackage[scale=.95,type1]{cabin}
\usepackage[zerostyle=c,scaled=.94]{newtxtt}
\usepackage[T1]{fontenc} 
\usepackage[utf8]{inputenc} 
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsaddr}
\usepackage{xspace,subcaption}
\usepackage{enumitem} 
\usepackage{csquotes}
\usepackage{xcolor,array}
\usepackage{tabularx}
\usepackage[colorlinks]{hyperref}
\pdfstringdefDisableCommands{\def\eqref#1{(\ref{#1})}}
\hypersetup{colorlinks, breaklinks, citecolor=teal,filecolor=black}
\RequirePackage[capitalize,nameinlink]{cleveref}[0.19]
\newcommand{\crefrangeconjunction}{--}
\crefformat{equation}{\textup{#2(#1)#3}}
\usepackage{graphicx}
\usepackage{mathtools}
\usepackage{pgfplots,tikz}
\pgfplotsset{compat=1.17}
\mathtoolsset{centercolon}
\usepackage{bm}
\usepackage{pgfkeys}
\usepackage{pgf,interval}
\intervalconfig{soft open fences}
\usepackage{asymptote}
\begin{asydef}
    import graph;
    import contour;
    import palette;
    size(3.8cm,3.8cm,IgnoreAspect);
    int N=200; 
    int Levels=10;
    pen[] Palette=Gradient(Levels,RGB(100,100,255),RGB(255,100,100));
    defaultpen(fontsize(8pt));
    pair tauC(real t) {
        if (t < 1/3) { return (t/sqrt(3),-t); }
        if (t < 2/3) { return (1/sqrt(27)+(t - 1/3)*(3 - 2/sqrt(3)),-1/3 );  }
        return (1-(1-t)/sqrt(3),-(1-t));
    }
    real ff(pair a, real ee, pair tau, real eta) {
        return xpart( - ee*a + 0.5*log(1+2*a+a*a*tau)-log(a)-0.5*log(tau)-(1+a-2*eta^2 * a^2 * (1 - tau))/(1+2*a+a*a*tau)  ) ;
    }
    real sc(real ee, pair tau, real eta) {
        if(ee<abs(tau)) { return ee^(-1/3)*(1/2+abs(tau)^(-2/3)/2 ); }
        if(eta<sqrt(ee)) {return ee^(-1)/2;}
        return abs(tau)^(-1)/2;
    }
    real sc(real ee, pair tau, real eta) {
        return max( (min(eta^2/ee,ee^(-1/3))-1)/abs(tau), ee^(-1/3)/2 + min(1/ee,ee^(-1/3)*abs(tau)^(-2/3))/2 );
    } 
    pair aCu(real t) {
        if(t<1) { return t*(cos(pi/6),sin(pi/6)); }
        return (cos(pi/6),sin(pi/6)) + (t-1)*(cos(3*pi/5),sin(3*pi/5));
    }
    real phiC = .5/sin(pi/6-3*pi/5)*(sqrt(3)*cos(3*pi/5) - sin(3*pi/5));
    pair aC(real r, real t) {
        return phiC*r*aCu(t);
    }
\end{asydef}
